Reproducibility Companion Paper: Swarical: An Integrated Hierarchical Approach to Localizing Flying Light Specks

This companion paper provides artifacts and instructions on replicating the experiments in the ACM Multimedia 2024 paper entitled "Swarical: An Integrated Hierarchical Approach to Localizing Flying Light Specks." Swarm-based hierarchical, Swarical, is a localization technique that enables miniature drones, Flying Light Specks (FLSs), to accurately and efficiently localize and illuminate complex 2D and 3D shapes. It consists of two components, an offline planner and an online localization technique that executes on an FLS. The offline planner uses the FLS sensor specification for positioning to convert mesh files into swarms of FLSs. Some FLSs are dark and used only for localization. We reported the online localization technique to be fast and highly accurate. We describe how to reproduce this finding using our artifacts.

==> experimetns.tex <==
In this section, we describe the experiments of the original paper.



\subsection{Environment}
The following requirements are needed to conduct the experiments.

\begin{itemize}
    \item Python3 with virtual environment. The software is tested with Python 3.10 on MacOS and Ubuntu 20 LTS. The required packages and instructions on setting up the virtual environment and installing the packages are available under the "Setup and Install Requirements" section of the \texttt{README} file from the GitHub repository.
    \item Access to a cloud service to reproduce large-scale results. We have tested Amazon Web Services and CloudLab. Instructions are available in \texttt{AWS\_README} and \texttt{CloudLab\_README} files.
\end{itemize}

\subsection{Components}



The GitHub repository contains two main components: planner (offline) and decentralized localization (online). The planner is run before the online component and provides the required data structures for the online component; see Figure\ref{fig:planner}. 



\subsection{Offline: Planner Experiments}
Here, we describe the features of the planner and show how to reproduce its results. \texttt{reproduction.ipynb} Jupyter Notebook walks you through running planner experiments. It also provides a means of analyzing and visualizing the results. These experiments produce data structures required by the FLS experiments. 

\subsection{Online: FLS Experiments}

% \begin{table}[]
%     \centering
%     \caption{Experimental parameters of online component.}
    
%     \begin{tabular}{c c c c}
%     \hline
%          Name & Description & Default Value & Type \\
%          \hline
%          DEAD_RECKONING_ANGLE & & & \\
%          ACCELERATION & & & \\
%          DECELERATION & & & \\
%          MAX_SPEED & & & \\
%          DURATION
%          SHAPE
%          CAMERA
%          SS_ERROR_MODEL
%          GROUP_TYPE
%     \end{tabular}

%     \label{tab:params}
% \end{table}

FLS experiments are the experiments that emulate FLSs with Python processes. Swarical launches one FLS process per point in the point cloud. Each process implements FLS movement, communication, and decentralized localization. These experiments require at least one processing core per FLS process. With point clouds with a few points, it is possible to run the experiments on a local machine. With a larger number of points, experiments require scaling across multiple machines. We used a cluster of 20 Amazon AWS servers, c6a.metal, with 192 virtual cores to conduct experiments with the Skateboard point cloud, which has 1372 FLSs plus 40 standby FLSs.

\subsubsection{Small-scale Experiments}\label{sec:small_exp}
We generate small point clouds with a 2D grid arrangement of points to test the decentralized algorithms locally. The example code for generating the point cloud and conducting a small-scale experiment is in the Decentralized Localization section of the \texttt{reproduction.ipynb} notebook of the Swarical GitHub repository. After performing the experiment, you can visualize the movement of the FLSs during localization as a video.

\subsubsection{Large-scale Experiments}
Large-scale experiments are online experiments using AWS with large point clouds. The required data structures should be generated using the planner before starting the experiments. Generate Trees for All Shapes section of the \texttt{reproduction.ipynb} notebook generates all the required files. The instructions on how to run the large-scale experiments are presented in \texttt{AWS\_README}. The provided scripts deploy and set up the software on each node of the cluster to conduct a list of experiments. The list of experiments is generated based on the user-defined varying configurations. The varying configurations are listed in the \texttt{gen\_cong.py} file, and the scripts generate one configuration file for each experiment and run the experiments consequently. The existing \texttt{gen\_cong.py} generates the original experiments of the Swarical paper. The raw results of these experiments include the flight path of each FLS and messages sent and received by each FLS. After postprocessing the raw results according to the \texttt{AWS\_README} file, use the \texttt{reproduction.ipynb} notebook to generate the animation visualization, presented in the caption of Figure 13 of the original paper (\m{\href{https://youtu.be/GncnoqqYT_w}{ISR}}, \m{\href{https://youtu.be/0_Gs7IkDADw}{HC}}, and \m{\href{https://youtu.be/YlLCxW32tvg}{RSF}}). Use the \texttt{swaricalplots.nb} to generate Figures 13, 14, and 15 of the paper. There is a link in the notebook to an archive containing the original raw results of the experiments that we reported in the original paper.

In addition to AWS, we provide instructions and scripts to run experiments of CloudLab; see \texttt{CloudLab\_README}. Depending on the available servers and the cluster's total number of processing cores, you can experiment with a small or large point cloud. An example of a small point cloud is the chess piece with 100 points available in the dataset. Grid point clouds with fewer or more points can also be generated and used.


==> reproOLD.tex <==

Our reproducibility study encompassed three experimental setups, using the public codebase that the author released. 

First, we re-executed the small-scale experiments responsible for the paper’s illustrative figures on mid-range Linux servers.
A subset of 3D meshes required minor, author-supplied code patches,
and an early race condition in the parallel execution code produced transient error logs until corrected.
Ultimately, all figures were successfully regenerated.
Second, the large-scale experiments were also reproduced without numerical deviation, but only after a protracted installation and configuration process on a cloud instance with large distributed computational power; this stage would include non-negligible economic costs. 

Lastly, we re-conducted a subset of the experiments
to quantify the error in visual pose estimation using ArUco fiducial markers.
This took time because it required 
obtaining various hardware components,
printing 3D models to reconstruct the experimental setup,
and then re-conducting the experiment.
The exact hardware used in the original paper was unavailable during the reproduction.
We only had available a Raspberry Pi camera module 3 with a wide-angle lens and
\emph{with} IR filter, whereas the original paper tested both wide-angle and regular lenses
-- both \emph{without} IR filters.
After clarifying several aspects of the experimental setup with the authors,
we reproduced 4 of 5 experiments done with the wide-angle lens camera in the original paper,
obtaining similar results with only small variations (likely due to manufacturing inconsistencies).
Sharing the process via video, in addition to reading the paper, was crucial to accurately converging on the
correct methodology. The paper and documentation has correspondingly been updated.

